Enabling Deep Reinforcement Learning on Energy Constrained Devices at the Edge of the Network

Deep Reinforcement Learning (DRL) solutions are becoming pervasive at the edge of the network as they enable autonomous decision-making in a dynamic environment. However, to be able to adapt to the ever-changing environment, the DRL solution implemented on an embedded device has to continue to occasionally take exploratory actions even after initial convergence. In other words, the device has to occasionally take random actions and update the value function, i.e., re-train the Artificial Neural Network (ANN), to ensure its performance remains optimal. Unfortunately, embedded devices often lack processing power and energy required to train the ANN. The energy aspect is particularly challenging when the edge device is powered only by a means of Energy Harvesting (EH). To overcome this problem, we propose a two-part algorithm in which the DRL process is trained at the sink. Then the weights of the fully trained underlying ANN are periodically transferred to the EH-powered embedded device taking actions. Using an EH-powered sensor, real-world measurements dataset, and optimizing for Age of Information (AoI) metric, we demonstrate that such a DRL solution can operate without any degradation in the performance, with only a few ANN updates per day.

==> tikz_figures/main_results_bigger_value.tex <==
\begin{tikzpicture}

\begin{groupplot}[group style={group name=my_plots, group size=3 by 3,vertical sep= 1.75cm}, width=0.45\textwidth,height=0.25\textwidth,]]

%\begin{groupplot}[group style={group name=my_plots, group size=3 by 3,vertical sep= 2cm, horizontal sep= 2.5cm}, width=0.65\textwidth,height=0.35\textwidth,]]

\nextgroupplot[
axis lines=middle,
title = (a) Average AoI for Low Profile,
xlabel=Capacity(F),
%ylabel=$\mathbb{E} \overbrace{a} \mathcal{L} $(years),
ylabel=Average AoI (min),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
ytick ={1800, 3600, 5400, 7200, 9000, 10800,12600, 14400 },
yticklabels={30,60,90,120,150, 180, 210},
scaled y ticks = false,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(2.2,1.5)}, legend columns=-1},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 16000,
every tick/.style={
	black,
	semithick,
}]
\draw[black!60,dashed] (0,420) -- (435, 420);
\draw[black!60,dashed] (0,360) -- (435, 360);
\draw[black!60,dashed] (0,300) -- (435, 300);
\draw[black!60,dashed] (0,126) -- (435, 126);
\draw[black!60,dashed] (0,90) -- (435, 90);
\draw[black!60,dashed] (0,54) -- (435, 54);
\draw[black!60,dashed] (0,18) -- (125, 18);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=avg_aoi,col sep=comma]{csv_data/uni_low.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=avg_aoi,col sep=comma]{csv_data/random_low.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=avg_aoi,col sep=comma]{csv_data/thold_low.csv};
%\addplot[style=loosely dotted, mark size=2pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=avg_aoi,col sep=comma]{csv_data/learn_low.csv};
%\addplot[blue, line width=1pt, mark=*] %
%table[x=days,y=avg_aoi,col sep=comma]{csv_data/random_4F.csv};


\addlegendentry{Ideal};
\addlegendentry{Random};
\addlegendentry{Threshold};
\addlegendentry{Deep RL};

%\addplot table [x=density,y=energy, col sep=comma] {csv_data/our_approach.csv};

%\addplot[line width=0.5pt,dotted,color=red]%
%table[x=days,y=avg_aoi,col sep=comma]{csv_data/learn_4F.csv};

%\addplot[line width=0.5pt,dashed,color=green] %
%table[x=density,y=worst,col sep=comma]{csv_data/clustering.csv};

\nextgroupplot[
axis lines=middle,
title = (b) Peak AoI for Low Profile,
xlabel=Capacity(F),
ylabel= Peak AoI (h/day),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
ytick ={3600, 10800, 18000, 25200, 32400, 39600, 46800},
yticklabels={1,3,5,7,9,11,13},
scaled y ticks = false,
%xtick={10,20,30,40,50},
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(0.40,0.40)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 55000,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (0,468) -- (435, 468);
\draw[black!60,dashed] (0,396) -- (435, 396);
\draw[black!60,dashed] (0,324) -- (435, 324);
\draw[black!60,dashed] (0,252) -- (435, 252);
\draw[black!60,dashed] (0,180) -- (435, 180);
\draw[black!60,dashed] (0,108) -- (435, 108);
\draw[black!60,dashed] (0,36) -- (435, 36);


\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=avg_peak,col sep=comma]{csv_data/uni_low.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=avg_peak,col sep=comma]{csv_data/random_low.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=avg_peak,col sep=comma]{csv_data/thold_low.csv};

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=avg_peak,col sep=comma]{csv_data/learn_low.csv};

%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};


\nextgroupplot[
axis lines=middle,
title = (c) Down-time for Low Profile,
xlabel=Capacity(F),
ylabel= $T_{down}$ (h),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
ytick ={600, 1200, 1800, 2400, 3000, 3600, 4200, 6000, 6600, 7200},
yticklabels={1,2,3,4,5,6,7,10,11,12},
%xtick={10,20,30,40,50},
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(0.40,0.40)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 8500,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (0,720) -- (435, 720);
\draw[black!60,dashed] (0,660) -- (435, 660);
\draw[black!60,dashed] (0,600) -- (435, 600);
\draw[black!60,dashed] (0,420) -- (435, 420);
\draw[black!60,dashed] (0,360) -- (435, 360);
\draw[black!60,dashed] (0,300) -- (435, 300);
\draw[black!60,dashed] (0,240) -- (435, 240);
\draw[black!60,dashed] (0,180) -- (435, 180);
\draw[black!60,dashed] (0,120) -- (435, 120);
\draw[black!60,dashed] (0,60) -- (435, 60);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=down_t,col sep=comma]{csv_data/uni_low.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=down_t,col sep=comma]{csv_data/random_low.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=down_t,col sep=comma]{csv_data/thold_low.csv};

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=down_t,col sep=comma]{csv_data/learn_low.csv};

%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};


\nextgroupplot[
axis lines=middle,
title = (a) Average AoI for Medium Profile,
xlabel=Capacity(F),
%ylabel=$\mathbb{E} \overbrace{a} \mathcal{L} $(years),
ylabel=Average AoI (min),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
ytick ={600, 1200, 1800, 2400, 3000, 3600, 4200},
yticklabels={10,20,30,40,50,60,70},
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(1,1)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 4000,
every tick/.style={
	black,
	semithick,
}]
%\draw[black!60,dashed] (0,420) -- (435, 420);
%\draw[black!60,dashed] (0,360) -- (435, 360);
\draw[black!60,dashed] (0,300) -- (435, 300);
\draw[black!60,dashed] (0,240) -- (435, 240);
\draw[black!60,dashed] (0,180) -- (435, 180);
\draw[black!60,dashed] (0,120) -- (435, 120);
\draw[black!60,dashed] (0,60) -- (125, 60);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=avg_aoi,col sep=comma]{csv_data/uni.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=avg_aoi,col sep=comma]{csv_data/random.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=avg_aoi,col sep=comma]{csv_data/thold.csv};
%\addplot[style=loosely dotted, mark size=2pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=avg_aoi,col sep=comma]{csv_data/learn.csv};
%\addplot[blue, line width=1pt, mark=*] %
%table[x=days,y=avg_aoi,col sep=comma]{csv_data/random_4F.csv};


%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};

%\addplot table [x=density,y=energy, col sep=comma] {csv_data/our_approach.csv};

%\addplot[line width=0.5pt,dotted,color=red]%
%table[x=days,y=avg_aoi,col sep=comma]{csv_data/learn_4F.csv};

%\addplot[line width=0.5pt,dashed,color=green] %
%table[x=density,y=worst,col sep=comma]{csv_data/clustering.csv};

\nextgroupplot[
axis lines=middle,
title = (b) Peak AoI for Medium Profile,
xlabel=Capacity(F),
ylabel= Peak AoI (min/day),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
ytick ={1800, 5400, 9000, 12600, 16200, 19800 },
yticklabels={30,90,150,210, 270, 330},
%xtick={10,20,30,40,50},
xtick={2,4,6,8,10},
scaled y ticks = false,
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(0.40,0.40)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 23000,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (50,198) -- (435, 198);
\draw[black!60,dashed] (0,162) -- (435, 162);
\draw[black!60,dashed] (0,126) -- (435, 126);
\draw[black!60,dashed] (0, 90) -- (435, 90);
\draw[black!60,dashed] (0, 54) -- (435, 54);
\draw[black!60,dashed] (0, 18) -- (435, 18);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=avg_peak,col sep=comma]{csv_data/uni.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=avg_peak,col sep=comma]{csv_data/random.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=avg_peak,col sep=comma]{csv_data/thold.csv};

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=avg_peak,col sep=comma]{csv_data/learn.csv};

%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};


\nextgroupplot[
axis lines=middle,
title = (c) Down-time for Medium Profile,
xlabel=Capacity(F),
ylabel= $T_{down}$ (h),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
ytick ={600, 1200, 1800, 2400, 3000, 3600},
yticklabels={1,2,3,4,5,6},
%xtick={10,20,30,40,50},
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(0.40,0.40)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 3800,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (25,360) -- (435, 360);
\draw[black!60,dashed] (0,300) -- (435, 300);
\draw[black!60,dashed] (0,240) -- (435, 240);
\draw[black!60,dashed] (0,180) -- (435, 180);
\draw[black!60,dashed] (0,120) -- (435, 120);
\draw[black!60,dashed] (0,60) -- (435, 60);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=down_t,col sep=comma]{csv_data/uni.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=down_t,col sep=comma]{csv_data/random.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=down_t,col sep=comma]{csv_data/thold.csv};

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=down_t,col sep=comma]{csv_data/learn.csv};

%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};



\nextgroupplot[
axis lines=middle,
title = (a) Average AoI for High Profile,
xlabel=Capacity(F),
%ylabel=$\mathbb{E} \overbrace{a} \mathcal{L} $(years),
ylabel=Average AoI (min),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
ytick ={300, 600, 900, 1200, 1500},
yticklabels={5,10,15,20,25},
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(1,1)}},
xmin=0.5, xmax=10.5,
ymin= 0, ymax= 1750,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (0,150) -- (435, 150);
\draw[black!60,dashed] (0,90) -- (435, 90);
\draw[black!60,dashed] (0,30) -- (435, 30);
\draw[black!60,dashed] (0,120) -- (435, 120);
\draw[black!60,dashed] (0,60) -- (125, 60);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=avg_aoi,col sep=comma]{csv_data/uni_high.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=avg_aoi,col sep=comma]{csv_data/random_high.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=avg_aoi,col sep=comma]{csv_data/thold_high.csv};
%\addplot[style=loosely dotted, mark size=2pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=avg_aoi,col sep=comma]{csv_data/learn_high.csv};
%\addplot[blue, line width=1pt, mark=*] %
%table[x=days,y=avg_aoi,col sep=comma]{csv_data/random_4F.csv};


%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};

%\addplot table [x=density,y=energy, col sep=comma] {csv_data/our_approach.csv};

%\addplot[line width=0.5pt,dotted,color=red]%
%table[x=days,y=avg_aoi,col sep=comma]{csv_data/learn_4F.csv};

%\addplot[line width=0.5pt,dashed,color=green] %
%table[x=density,y=worst,col sep=comma]{csv_data/clustering.csv};

\nextgroupplot[
axis lines=middle,
title = (b) Peak AoI for High Profile,
xlabel=Capacity(F),
ylabel= Peak AoI (min/day),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
scaled y ticks = false,
ytick ={1800, 5400, 9000},
yticklabels={30,90,150},
%xtick={10,20,30,40,50},
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(0.40,0.40)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 13000,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (50,360) -- (435, 360);
\draw[black!60,dashed] (0,300) -- (435, 300);
\draw[black!60,dashed] (0,240) -- (435, 240);
\draw[black!60,dashed] (0,90) -- (435, 90);
\draw[black!60,dashed] (0,54) -- (435, 54);
\draw[black!60,dashed] (0,18) -- (435, 18);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=avg_peak,col sep=comma]{csv_data/uni_high.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=avg_peak,col sep=comma]{csv_data/random_high.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=avg_peak,col sep=comma]{csv_data/thold_high.csv};

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=avg_peak,col sep=comma]{csv_data/learn_high.csv};

%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};


\nextgroupplot[
axis lines=middle,
title = (c) Down-time for High Profile,
xlabel=Capacity(F),
ylabel= $T_{down}$ (h),
%width=0.75\linewidth,
%height=0.5\linewidth,
%font=\tiny,
%tick align=outside,
%xtick pos = left,
%ytick pos = left,
font=\small,
ytick ={600, 1200, 1800, 2400},
yticklabels={1,2,3,4,5,6},
%xtick={10,20,30,40,50},
xtick={2,4,6,8,10},
xticklabels={2,4,6,8,10},
%xticklabels from table={csv_data/equal_data_rate_tikz.dat}{Label},
%xticklabel style={align=center},
%legend pos=south west,
legend style={at={(0.40,0.40)}},
xmin=0.5, xmax=10.5,
ymin= 0,ymax= 2700,
every tick/.style={
	black,
	semithick,
}]

\draw[black!60,dashed] (25,240) -- (435, 240);
\draw[black!60,dashed] (0,180) -- (435, 180);
\draw[black!60,dashed] (0,120) -- (435, 120);
\draw[black!60,dashed] (0,60) -- (435, 60);

\addplot[style=loosely dotted, mark size=1pt, line width=1pt, color=blue!90, mark=otimes*, smooth, mark options={solid}]
    table[x=cap,y=down_t,col sep=comma]{csv_data/uni_high.csv};

\addplot[mark size=2pt, line width=1pt, color=blue!30, mark=triangle*, mark options={solid}]
    table[x=cap,y=down_t,col sep=comma]{csv_data/random_high.csv};

\addplot[style=dotted,mark size=2pt, line width=1pt, color=blue!60, mark=square*, smooth, mark options={solid}]
     table[x=cap,y=down_t,col sep=comma]{csv_data/thold_high.csv};

\addplot[style=loosely dashed, mark size=2pt, line width=1pt, color=red!75, mark=pentagon*, smooth, mark options={solid}]
table[x=cap,y=down_t,col sep=comma]{csv_data/learn_high.csv};

%\addlegendentry{Ideal};
%\addlegendentry{Random};
%\addlegendentry{Threshold};
%\addlegendentry{Deep RL};


\end{groupplot}
\end{tikzpicture}
